Pressure distribution of the high-redshift cluster of galaxies CL J1226.9+3332 with NIKA

The thermal Sunyaev-Zel'dovich (tSZ) effect is expected to provide a low scatter mass proxy for galaxy clusters since it is directly proportional to the cluster thermal energy. The tSZ observations have proven to be a powerful tool for detecting and studying them, but high angular resolution observations are now needed to push their investigation to a higher redshift. In this paper, we report high angular (< 20 arcsec) resolution tSZ observations of the high-redshift cluster CL J1226.9+3332 (z=0.89). It was imaged at 150 and 260 GHz using the NIKA camera at the IRAM 30-meter telescope. The 150 GHz map shows that CL J1226.9+3332 is morphologically relaxed on large scales with evidence of a disturbed core, while the 260 GHz channel is used mostly to identify point source contamination. NIKA data are combined with those of Planck and X-ray from Chandra to infer the cluster's radial pressure, density, temperature, and entropy distributions. The total mass profile of the cluster is derived, and we find $M_{500} = 5.96^{+1.02}_{-0.79} $ x $10^{14} M_{\odot}$ within the radius $R_{500} = 930^{+50}_{-43}$ kpc, at a 68% confidence level. ($R_{500}$ is the radius within which the average density is 500 times the critical density at the cluster's redshift.) NIKA is the prototype camera of NIKA2, a KIDs (kinetic inductance detectors) based instrument to be installed at the end of 2015. This work is, therefore, part of a pilot study aiming at optimizing tSZ NIKA2 large programs.

==> Makefile <==
FICHIER_TEX= NIKA_CL1227.tex
FICHIER_BIB= biblio.bib
ARCHIVE=$(FICHIER_TEX:%.tex=%.zip)


all : 
	pdflatex ${FICHIER_TEX}
	bibtex $(FICHIER_TEX:%.tex=%)
	pdflatex ${FICHIER_TEX}
################################################
#lance le make de chaque sous rep
figltex : 
	grep includegraphics *.tex > liste.txt
	awk  '{st=index($$0,"{");rem=substr($$0,st+1); st=index(rem,"}"); rem=substr(rem,1,st-1); printf("pdf2ps  %s.pdf %s.ps\nconvert %s.png %s.ps\nps2eps %s.ps\nrm %s.ps\n",rem,rem,rem,rem,rem,rem);}' liste.txt > conv_liste.sh
	bash conv_liste.sh

ltex : 
	latex ${FICHIER_TEX}
	bibtex $(FICHIER_TEX:%.tex=%)
	dvips $(FICHIER_TEX:%.tex=%.dvi)
	ps2pdf $(FICHIER_TEX:%.tex=%.ps)

clean: $(REP)
	@echo "suppression des fichiers de compilation"
	@# fichiers de compilation latex
	@rm -f *.log *.aux *.dvi *.toc *.lot *.lof *.out
	@# fichiers de bibtex
	@rm -f *.bbl *.blg
	@# fichier zip 
	@rm -f *.zip

zip: 
	#rm ${ARCHIVE}
	grep includegraphics *.tex > liste.txt
	awk  '{st=index($$0,"{");rem=substr($$0,st+1); st=index(rem,"}"); rem=substr(rem,1,st-1); printf("zip -r ${ARCHIVE} %s.p*\nzip -r ${ARCHIVE} %s.j*\n",rem,rem);}' liste.txt > zip_liste.sh
	zip -r ${ARCHIVE} Makefile
	zip -r ${ARCHIVE} *.cls
	zip -r ${ARCHIVE} *.tex
	bash zip_liste.sh

zipltex:
	#rm ${ARCHIVE}
	grep includegraphics *.tex > liste.txt
	awk  '{st=index($$0,"{");rem=substr($$0,st+1); st=index(rem,"}"); rem=substr(rem,1,st-1); printf("zip -r ${ARCHIVE} %s.eps\n",rem);}' liste.txt > zip_liste.sh
	zip -r ${ARCHIVE} ${FICHIER_BIB}
	zip -r ${ARCHIVE} Makefile
	zip -r ${ARCHIVE} ${FICHIER_TEX}
	bash zip_liste.sh

